Federated Graph Learning with Structure Proxy Alignment

Federated Graph Learning (FGL) aims to learn graph learning models over graph data distributed in multiple data owners, which has been applied in various applications such as social recommendation and financial fraud detection. Inherited from generic Federated Learning (FL), FGL similarly has the data heterogeneity issue where the label distribution may vary significantly for distributed graph data across clients. For instance, a client can have the majority of nodes from a class, while another client may have only a few nodes from the same class. This issue results in divergent local objectives and impairs FGL convergence for node-level tasks, especially for node classification. Moreover, FGL also encounters a unique challenge for the node classification task: the nodes from a minority class in a client are more likely to have biased neighboring information, which prevents FGL from learning expressive node embeddings with Graph Neural Networks (GNNs). To grapple with the challenge, we propose FedSpray, a novel FGL framework that learns local class-wise structure proxies in the latent space and aligns them to obtain global structure proxies in the server. Our goal is to obtain the aligned structure proxies that can serve as reliable, unbiased neighboring information for node classification. To achieve this, FedSpray trains a global feature-structure encoder and generates unbiased soft targets with structure proxies to regularize local training of GNN models in a personalized way. We conduct extensive experiments over four datasets, and experiment results validate the superiority of FedSpray compared with other baselines. Our code is available at https://github.com/xbfu/FedSpray.

==> table_epoch.tex <==
\begin{table}[t]
\caption{Classification accuracy of FedSpray and Fedavg on node classification over WikiCS with GCN.}
\label{table:epoch}
\setlength\tabcolsep{10pt}
\begin{tabular}{cccc}
\hlineB{2}
\textbf{Epochs}                  & \textbf{Node sets}     & \textbf{FedAvg}                & \textbf{FedSpray}                  \\ \hline     
\multirow{2}{*}{$E=3$}  & Overall       & $80.38 \pm 0.85$      & $81.37 \pm 0.39$          \\
                        & Minority      & $35.04 \pm 2.79$      & $47.43 \pm 1.39$          \\ \hline
\multirow{2}{*}{$E=5$}  & Overall       & $80.53 \pm 0.74$      & $81.51 \pm 0.45$          \\
                        & Minority      & $35.48 \pm 2.52$      & $47.43 \pm 1.31$          \\ \hline
\multirow{2}{*}{$E=10$} & Overall       & $80.23 \pm 0.70$      & $81.43 \pm 0.51$          \\
                        & Minority      & $35.13 \pm 2.47$      & $46.85 \pm 1.18$          \\ 
\hlineB{2}

\end{tabular}
\end{table}


